The Sustainability Assessment Framework Toolkit: A Decade of Modeling Experience

Software intensive systems play a crucial role in most, if not all, aspects of modern society. As such, both their sustainability and their role in supporting sustainable processes, must be realized by design. To this aim, the architecture of software intensive systems should be designed to support sustainability goals; and measured to understand how effectively they do so. In this paper, we present the Sustainability Assessment Framework (SAF) Toolkit -- a set of instruments we developed to support software architects and design decision makers in modeling sustainability as a software quality property. The SAF Toolkit is the result of our experience gained in over a decade of cases in collaboration with industrial partners. We illustrate the toolkit with examples stemming from various cases. We extract our lessons learned, and our current research and future plans to extend the SAF Toolkit for further architecture modeling and measurement.

==> old/01_intro.tex <==
\section{Introduction}\label{sec:introduction}
% \assignedto{Patricia}

% role of software in all sectors
% role of software for sustainability by design
Software intensive systems play a crucial role in most, if not all, aspects of modern society. As such, both their own sustainability and their role in supporting sustainable processes, must be realized \textit{by design}.

From an environmental perspective, the energy footprint of digital solutions is worrisome. For example, the Energy Efficiency Directive for Data Centers~\cite{EED2023}, reports that \textit{in the EU, from 2010 to 2018 data centre energy consumption increased by 42\% and is forecast to further increase by 28.2\% by 2030, representing about 3.2\% of  the  EU  final  electricity demand.  Reducing  the  energy  demand  of  ICT,  including  data  centres,  is  an important step in the target reduction of overall GHG emissions of 55\% by 2030 compared to 1990 levels}. Given that nowadays most software is to various degrees cloud based (\eg~\cite{cloudsoftware2023a, cloudsoftware2023b}), its energy efficiency is imperative. If we also consider the global adoption of AI-based solutions like generative AI~\cite{generative_ai}, there is growing evidence that the energy footprint of software will escalate in the coming years~\cite{verdecchia2023systematic}.

Next to the environmental perspective, sustainability entails other dimensions which further increase the role of software in society at large: from a social perspective software usability, for example, can support or hinder accessibility to fundamental services like healthcare and education; from an economic perspective, affordability of software products and related technologies can significantly influence economic growth; and of course from a technical perspective, evolvability or integrability of software to accommodate over time the changes in society and consumer needs, can act as the motor for, or against, innovation.

% importance of architecture level
As sustainability and its dimensions have a broad scope and are interdependent, software professionals and decision makers need to consider software sustainability at a high level of abstraction. This way, the role of software elements and the way they influence one another can be (re-)designed for, monitored and reasoned about. The software architecture level provides the right abstraction needed for the above.

% focus on helping practitioners to embed sustainability in software early on
In this paper, we present the Sustainability Assessment Framework (SAF) Toolkit -- a set of instruments that aim to support software architects and design decision makers in modeling sustainability as a software quality property. The SAF Toolkit is the result of our experience gained in over a decade of cases in collaboration with industrial partners.

% intended audience
The \textbf{intended target audience} of this paper are (i) practitioners responsible both for setting priorities bringing software sustainability to the forefront of their organizations and for deciding on how sustainability concerns are designed in software solutions, and (ii) instructors willing to include software sustainability into Computer Science and Software Engineering programs. Both can access the SAF Toolkit guidelines, tutorials, and links to open-source instruments in the \textbf{supplementary online material}~\cite{saf_toolkit_online}.

We illustrate the toolkit with examples stemming from various cases \change{(the full list of cases is provided in \Cref{tab:cases})}. We extract our lessons learned, and our current research and future plans to extend the SAF Toolkit for further architecture modeling and measurement.

The remainder of this paper is organized as follows.
Section~\ref{sec:background} presents the background on the notion of sustainability, its relation to software as used in our work, and the notion of key performance indicator, while Section~\ref{sec:rw} presents related works.
Section~\ref{sec:toolkit} describes the SAF Toolkit and its instruments in detail, and explains the current release and its evolution over time, and the next steps for future research. 
Finally, in Section~\ref{sec:discussion} we discuss additional overarching observations, and conclude the paper.
% we elaborate on lessons learned for practitioners and instructors. 
% Finally, Section~\ref{sec:conclusion} summarizes the paper.


==> old/02_background.tex <==
\section{Background}\label{sec:background}
% \assignedto{Iffat/Markus}

In this section, we provide the background knowledge necessary for the remainder of this paper. We introduce the notion of sustainability in general and in the context of software. We provide an overview of sustainability in terms of the two dimensions that we find indivisible in a sound definition of sustainability, namely the dimension expressing the various sustainability aspects that are within the focus of a software intensive system, and the dimension expressing the related impact over time. We then close with the concept of Key Performance Indicator.

\subsection{Definition of Software Sustainability}
% \todo{Markus: on the definition of sustainability (Venters et al., 5Ws)}

In almost every sustainability research, regardless of the discipline, the definition of sustainability is repeatedly redefined without finding a common ground, resulting in a plethora of interpretations~\cite{CaleroEtAl_5WsGreen_2020, PetersEtAl_SustainabilityComputing_2024,CaleroPiattini_PuzzlingOut_2017}.
In software sustainability, \citet{VentersEtAl_SustainableSoftware_2023} %divide the research landscape in two eras: before and after the appearance of their initial article in 2018 about 
discuss the "maturity of software sustainability from a software architecture point of view". The authors conclude that there is no universally accepted definition of software sustainability for either era; software sustainability is either "a measure of endurance" or "aligned [...] to one or more software quality attributes". Nevertheless, in addition to technical and environmental aspects, the literature now recognizes other dimensions such as the economic, social, and individual ones~\cite{VentersEtAl_SustainableSoftware_2023} (see also \Cref{sec:dimensions}).

Due to this variety of definitions and the importance of software in an increasingly digitalized society, we see software sustainability as the software "ensuring that the intended benefits are preserved over time, notwithstanding who uses them or where they are deployed"~\cite{Lago_ConnectedWorld_2023}. For a more comprehensive understanding of sustainability, we encourage the interested reader to explore various in-depth examinations and definitions available on the subject, \eg~\cite{PetersEtAl_SustainabilityComputing_2024,BeckerEtAl_SustainabilityDesign_2015, CaleroEtAl_5WsGreen_2020, VentersEtAl_BlindMen_2014, CaleroEtAl_IntroductionSoftware_2021, AndrikopoulosEtAl_SustainabilitySoftware_2022,Heldal2024-industry}.



\subsection{The Dimensions of ``Sustainability Focus'' (or Sustainability Dimension)} \label{sec:dimensions}
% \todo{Markus: definition of dimensions of focus (4D, other classifications); direct and indirect impact (e.g. work of Calero)}

% \todo{if necessary, we can also include and compare the dimensions from Calero et al. (2021) as describe in the book "Software Sustainability", i.e., Environmental, Human, Economic.}

As previously stated, achieving sustainability involves various dimensions and finding a balance between them while also considering their trade-offs~\cite{LagoEtAl_FramingSustainability_2015}. 
At a higher abstraction level, the PESTLE model examines sustainability from Political, Economic, Social, Technological, Legal, and Environmental perspectives to identify challenges and opportunities for businesses~\cite{Nandonde_PESTLEAnalysis_2019}. The ESG framework focuses on a smaller subset of factors, namely Environmental, Social, and corporate Governance, which should be aligned to ensure sustainable investment in the financial market and international organisations~\cite{EuropeanBankingAuthority_ReportIncorporating_2022}.

Also in computer sciences, there are different perspectives on sustainability. 
The SAF with its focus on software architecture in particular reflects on the four sustainability dimensions according to \citet{LagoEtAl_FramingSustainability_2015}: (i) \textit{Technical} dimension encompasses implementation aspects, as well as concerns related to the evolution, maintenance, and long-term utilisation of software-intensive systems; (ii) \textit{Economic} dimension revolves around business considerations, such as capital investment and profitability; (iii) \textit{Social} dimension emphasises the integration of the systems within communities considering their impact on individuals and society; (iv) \textit{Environmental} dimension extends beyond greenhouse gas emissions and encompasses the broader impacts of software activities on the natural ecosystem. In requirements engineering, for instance, a fifth \textit{Individual} dimension has emerged as important for reflecting on an individual's well-being~\cite{DubocEtAl_RequirementsEngineering_2020}.

% removed. is already discussed in 2.3
%When discussing the minimisation or maximisation of particular software impacts, we need to specify the type of impact being referred to. \citet{Naumann_2011} categorises the consumed energy of software as a direct impact, while impacts resulting from the usage of a particular software are considered indirect impacts. The authors particularly highlight the social implications that arise indirectly from using a software project, such as changes in how social communities communicate after the introduction of social platforms. The SAF toolkit frames these impacts in three different levels: (i) \textit{Immediate} impacts, referring to immediately observable changes; (ii) \textit{Enabling} impacts, arising from use over time; and (iii) \textit{Systemic} impacts, referring to persistent changes and requirements such as economic structural changes~\cite{Lago2019}.



\subsection{The Dimension of "Time" (or Time Dimension)}
% \todo{Iffat: definition of time dimension (Hilty et al. and order of effects; stability; book chapter Network Institute; other?)}

Apart from the various sustainability dimensions, sustainability has another facet \ie \textit{time}. \citet{Hilty_2015} present a framework for ICT impacts on sustainability with a three-level model for the over-time effects of ICT: (i) Level 1 refers to the \textit{direct effects} of the production, use or disposal of ICT; (ii) Level 2 refers to the \textit{enabling effects} of ICT as induction, obsolescence, substitution and optimization effects; (iii) Level 3 refers to the\textit{ systemic effects} which are the long-term socio-economic effects that induce a behavioral or economic structural change. This can be viewed as both negative re-bound effects and positive cascading effects. \citet{Hilty_2015} also identify an inherent limitation of their framework as it mixes up the levels of abstraction and categories of effects. It is not clear how micro-level action across one dimension can lead to a macro-level impact without impacting other dimensions of sustainability. Hence, an isolated action cannot be considered to have a strictly positive or negative effect unless its macro-level impact is studied. As sustainability goals take a macro-level perspective, this phenomenon requires a macro-level analysis.
% Should we add an example here? 


The intended benefits of sustainability decisions must uphold with ever-evolving nature of the digital landscape. In view of this, \citet{Lago_ConnectedWorld_2023} defines sustainability as ``the preservation of the beneficial use of digital solutions, in a context that continuously changes". Accordingly, software must be viewed for its over-time impact on sustainability. 


\subsection{Key Performance Indicators}
%\todo{Iffat: definition of KPIs? (e.g., Parmenter, Iffat)}

To supplement micro- and macro-level support for sustainability impact assessment across the different levels of abstraction, Key Performance Indicators (KPIs) can provide a solution by aggregating micro-level \textit{data} to macro-level \textit{indicators} to monitor sustainability concerns. 

Parmenter defines a KPI as ``an indicator that focuses on the aspects of organizational performance that are the most critical for the current and future success of the organization" \cite{Parmenter_2015}. To formalize KPIs for software, \citet{Fatima_2023} revise Parmenter's definition to ``an indicator that focuses on the aspects of \textit{software} performance that are the most critical for the current and future success of the organization''. By focusing on software performance aspects and linking it with organizational success, a KPI enables integrating software quality into organizational strategy as an intrinsic mechanism. Thus, KPIs act as a linchpin between the business and the technical ends of digital organizations for monitoring success. It is important to note that the word ‘performance’ in KPI does not refer to the quality attribute performance, but rather it means how well the software satisfies the critical success factors through its operation.

In the context of software, \citet{Staron_2016} define a KPI as ``a critical element in the transformation of raw data (numbers) into decisions (indicators)''. For example, in a later work~\cite{Staron_2012} they present a release readiness KPI to check when a product will be ready for release based on the number of defects present, defects removed and predicted defect discovery. A decision criteria is established based on thresholds or patterns. If the values deviate from a threshold or pattern, the KPI monitoring enables the quality manager to make decisions to trigger actions for improvement. The same concept can be applied to the field of software architecture by modeling software quality through KPIs, their targets representing the achievement of a design concern and by using these KPIs to drive architectural design decisions through actions.

==> old/03_related_work.tex <==
\section{Related Work}\label{sec:rw} 

In this section, we discuss the related works that focus on modeling frameworks or assessment initiatives aimed at achieving software sustainability. 

\citet{Naumann_2011} present a reference model for Green and Sustainable Software -- the GREENSOFT model. This model is designed to capture sustainability effects (first-, second-, and third-order of effects) of software from their inception until their end-of-life. The model is supplemented by metrics for sustainability criteria (common, direct and indirect). The model also provides procedure models for the development, purchase, operation and use of software in a sustainably-sound manner. It rounds off by providing recommendations and tools for software development, purchase, administration and usage. The GREENSOFT model focuses on both Green IT and Green by IT. 

\citet{Cabot_2009} use the i* framework for integration of sustainability design concerns in (i) design alternative selection for software, and (ii) decisions for business activities. The use of this framework is demonstrated through a case study by identifying sustainability-specific soft goals, tasks, agents and roles. Dependencies and relationships are identified between these elements. Goals are linked to each other with the relation of positive (`help') or negative (`hurt') impacts. The study acknowledges the challenges of the proposed approach as (i) difficulty in determining the appropriate level of detail for effectively representing sustainability, (ii) the need for a qualitative approach incorporating measurable measures to enhance the usefulness of the analysis, (iii) loose semantics of the proposed model, leading to consistency issues when different people use it, and (iv) lack of validation mechanism with stakeholder involvement for validation of decisions and their impacts. 

\citet{Penzenstadler_2013} present a meta-model that is instantiated as a sustainability model to analyze sustainability dimensions, value indicators, and support activities. The meta-model describes the sustainability dimension as an aspect of the goal. Indicators are used to quantify a value that represents certain sustainability dimensions. These indicators, guided by external regulations, guide the activities that lead to achieving sustainability. It is, however, challenging to identify possible conflicts between goals. To solve this issue, \citet{Saputri_2016} present an extension of this meta-model by including quality attributes as a measurement mechanism for indicators. A template is provided to carry out this trade-off analysis between goals by capturing the influence (conflict, support, neutral). 

\citet{Duboc_2020} present a framework to raise awareness on the sustainability impacts of software systems in the context of requirements engineering. They present a question-based Sustainability Awareness Framework (SusAF) supplemented by Sustainability Awareness Diagrams. This framework aims to facilitate discussions, for it to become a de-facto standard in the industry as a thinking tool for short, medium, and long-term sustainability impacts of socio-technical systems \cite{SusAF_Vision_2023}. 

More recently, the GAISSA project~\cite{GAISSA} provides architecture‐centric methods for the modeling and development of green AI‐based systems. It focuses on developing a greenability quality model for assessing AI models and systems, providing green-aware architecture-centric methods to data scientists and software engineers, and supporting analysis and decision-making for greenability improvement. 

\citet{GuldnerEtAl_DevelopmentEvaluation_2024a} provide a reference measurement model called the Green Software Measurement Model (GSMM). The model uses existing research to provide recommendations, processes, and tools to help evaluate and minimize software's environmental impact. The study presents a catalog of metrics to evaluate software's energy and resource consumption. Further, it provides a list of tools for automation, resource logging, analysis, and fully integrated solutions. Hence, GSMM aims to aid practitioners in developing and evaluating software products for resource and energy efficiency. 

\change{The frameworks and models found in the literature facilitate capturing and representing software sustainability in different stages of the Software Development Life Cycle. The existing frameworks either provide a high-level process view for monitoring but lack instruments for targeted decision making regarding specific elements of the  \cite{Naumann_2011, Cabot_2009, GuldnerEtAl_DevelopmentEvaluation_2024a}. Current research includes thinking frameworks that can aid in decision making but, with a focus on requirements \cite{Penzenstadler_2013, Duboc_2020, Saputri_2016}.  
We observe a missing link between goals and software measurement process, with software architecture at the center stage. Establishing a connection between micro-level metrics that represent sustainability of architectural elements to macro-level organizational sustainability goals, is essential for improvement and taking action. Determining the level of detail is a challenge observed in all frameworks as low-level details tend to get disconnected from high-level views of the systems and organizations. 
}

With the SAF Toolkit, we envision support along certain aspects, specifically in the context of software architecture by (i) measuring the Quality Requirements representing design concerns via metrics (already supported by the current release of the SAF Toolkit), (ii) establishing a link of design concerns to software architecture and its elements (partially supported by the SAF Toolkit), (iii) connecting the low-level metrics measuring the Quality Requirements with high-level goals represented by Key Performance Indicators (KPIs) (in the future release of SAF Toolkit). 

==> old/04-2_saf_in_action.tex <==
\section{\change{The SAF Toolkit in Action}}\label{sec:SAFinAction}

\change{In this section we outline how we envision the complete SAF Toolkit workflow for its intended stakeholders. Architects and decision makers can use this knowledge to understand how the toolkit could be integrated into their current work process; educators can use it as a teaching guide on what steps are necessary to address sustainability holistically in the software engineering process. As shown in \Cref{fig:SAFinAction}, we distinguish between two vision cycles.}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/SAF-in-action.pdf}
    \caption{\change{\textbf{SAF Toolkit in Action divided in two vision cycles.} The gray phases in the \textit{Design Cycle} are available in the current version; the dashed phases in the \textit{Monitoring Cycle} are plan of our future vision and have yet to be integrated.}}
    \label{fig:SAFinAction}
\end{figure}

\change{
The \textbf{Design Cycle} focuses on the incremental design of the DM (01), the SQ model (02) and the use of the KPI template (03).  In this iterative process, the Checklist and Decision Graph (see \Cref{sec:guidingInstrument}) are used as instruments to guide the creation of a comprehensive DM.  
The Dependency Matrices (see \Cref{sec:DMatrix}) support the decision making process by revealing the relationships between the identified QAs in the DM and SQ Model. The matrices can also be refined and extended during the design process to suit the needs of the context and the experience gained. 
We expect the Design Cycle to be completed by formulating KPIs accordingly. The cycle will be re-initiated with evidence-based feedback (07) from the Monitoring Cycle.
}

\change{
The \textbf{Monitor Cycle} is concerned with activities that are applied and executed at the system's runtime. In order to facilitate the feedback from the implemented system back to the Design Cycle, it is necessary to establish a mapping of Architecture Elements (04), integrate the Green Lab (05), and employ certain Monitoring Dashboards (06). 
By mapping architectural features, decisions, and concerns to concrete architectural elements in the software architecture as described in \Cref{sec:SAF+SA}, we can identify which metrics should be measured where.
This understanding is essential for the Green Lab to collect concrete measures from an implemented architecture. Monitoring Dashboards would gather the measured evidence and feed them back to the Design Cycle.
}

==> old/04_saf_toolkit.tex <==
\section{The {SAF} Toolkit}\label{sec:toolkit}
%this describes each tool, uses one example, and presents the related lesson learned

To provide a thorough introduction to the SAF Toolkit, we organize this section in three parts. First, we take a bird's eye view of the toolkit to understand all instruments involved and how they interact. Then, we zoom into each instrument individually to examine their elements and show how the instrument has evolved over time to the current release of the toolkit. Finally, we outline our plan for the future and how we envision the planned extensions.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The Big Picture}\label{sec:bigpicture}
% overview of SAF 

\Cref{fig:structuralModel} provides an overview of all the instruments that are part of the SAF Toolkit and those that are planned as future extensions. We refer to this view as the \textit{SAF Toolkit Overview}, as it presents the instruments at a high level of abstraction and illustrates their inter-relationships.

In its current release (see inside the dashed blue rectangle), the SAF Toolkit consists of its two main instruments, namely the Sustainability-Quality (SQ) Model and the Decision Map (DM), both adopting a shared definition of the sustainability dimensions. This definition is used to classify the quality requirements from the perspective of the sustainability dimension to which the quality requirements relate.

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/structuralView_small.pdf}
    \caption{\textbf{SAF Toolkit Overview}. High-level overview of all involved instruments and their relation. Instruments inside the dashed-blue rectangle are available in its current version; instruments outside are plan of our future vision and have yet to be integrated. The figure builds upon the notation for Unified Modeling Language (UML) defined in ISO/IEC 19501 \cite{ISO_19501_2005}.}
    \label{fig:structuralModel}
\end{figure}

In particular, to frame and illustrate sustainability-relevant design and quality requirements (QRs), the visual notation of \textbf{Decision Maps (DMs)} is utilized. DMs serve as a thinking framework to capture, reason, and uncover dependencies among sustainability-related QRs in the form of a visual diagram. Such visualization is also intended to foster communication among software architects regarding the sustainability of their software-intensive systems.

To consolidate definitions about the identified concerns, the \textbf{Sustainability-Quality (SQ) Model} encompasses a collection of Quality Attributes (QAs)\footnote{In the context of the SAF Toolkit, we use interchangeably terms \textit{quality requirement} and \textit{quality attribute} depending on the context of the discussion. This follows the observation by \citet{boer_vanvliet2009}, that quality requirements become quality attributes during the design phase of a given software project.} grouped into the four sustainability dimensions. QAs are derived in accordance with the ISO/IEC 25010 standard \cite{ISO_25010_2011} and are based on QAs identified in prior projects \cite{Condori-FernandezLago_CharacterizingContribution_2018, Condori-FernandezEtAl_ActionResearch_2020}. The SQ Model operationalizes the identified QAs provided by the DM by assigning a set of metrics and measures.

Research indicates that sustainability necessitates a careful assessment of trade-offs but within distinct \textbf{Sustainability Dimensions} \cite{LagoEtAl_FramingSustainability_2015, BetzEtAl_SustainabilityDebt_2015, Condori-FernandezLago_CharacterizingContribution_2018}. As mentioned in \Cref{sec:dimensions}, different disciplines feature varying types and numbers of dimensions. The SAF Toolkit, with its DM and SQ Model aligns with the four sustainability dimensions as proposed by \citet{LagoEtAl_FramingSustainability_2015}. Nonetheless, while all four dimensions should be taken into account during the design phase to achieve balance, it is not always necessary for every dimension to be relevant for a specific software system \cite{Condori-FernandezLago_CharacterizingContribution_2018}. 

\Cref{sec:SAFnow} delves deeper into the current release of the SAF Toolkit by further explaining each instrument.

The instruments yet to be integrated (see outside the dashed-blue rectangle in \Cref{fig:structuralModel}) include the KPI Model and the Software Architecture standard. To establish and define the metrics and measures for the QAs within the SQ Model in a systematic way, we aim to incorporate a \textbf{KPI Model}. Such a model will assist us in identifying sound KPIs relevant to the specific software project at hand. 
KPIs can emerge from two distinct approaches, top-down or bottom-up. 
In a top-down assessment, we envisage that KPIs can be formulated by starting with a sustainability goal derived from the DM, followed by gathering the relevant metrics and measures. 
Conversely, in a bottom-up assessment, concrete metrics from the SQ Model would be used to formulate, or associate to, a particular goal. 
Overall, once comprehensive KPIs are established in a systematic and traceable manner, they can provide essential feedback on QAs and related design decisions through tangible measures.

To contextualize the software architecture of a given software-intensive system, we aim to enhance the SAF Toolkit by positioning it with respect to the \textbf{Software Architecture ISO/IEC/IEEE 42010 Standard} \cite{ISO_42010_2022} and explicitly integrating the relevant architecture elements. If present, this integration would enable us to link the QAs from the DM with specific architecture elements, such as software services or components. This connection is crucial for (i) understanding where to measure the previously defined KPIs and consequently (ii) determining the impact of a specific architectural element on a particular QA. \\
The detailed conceptualization and integration for the planned extensions are elaborated upon in \Cref{sec:SAFfuture}.


% \assignedto{Markus}
% \todo{add overview figure}
% \todo{differentiate between current and future version; point to 4.2 and 4.3}
% \todo{describe instruments/elements}
% \todo{describe relations}

% historical overview of case studies:
% \assignedto{Patricia} \todo{table with case studies + coverage big picture elements}
%\assignedto{Patricia} \todo{comment on the overlap with the previous figures and the DM extensions}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{The SAF Toolkit: Where we are now}\label{sec:SAFnow}
% \assignedto{Patricia}
The current release of the SAF Toolkit produces two main outputs, the Decision Map and the SQ Model. To do so, the toolkit user is provided with a set of so-called instruments, \ie tools providing the necessary guidance. 

The following explains both outputs and for each of them, describes (i) the conceptual elements they frame, (ii) the visual elements with examples from some of our past projects, and (iii) the instruments guiding their creation. We close with a reflection on the experience and the points for improvement related to each instrument.

\begin{sidewaysfigure}[htbp!]
    \centering
    \includegraphics[width=1\linewidth]{figures/SAFModel_now+future_sm.pdf}
    \caption{\change{\textbf{SAF Toolkit Model}}. Detailed-level overview of all involved instruments, their elements and relation. Colored elements are available in its current version; Transparent elements are plan of our future vision and have yet to be integrated. The figure uses the notation for Unified Modeling Language (UML) defined in ISO/IEC 19501 \cite{ISO_19501_2005}. A more accessible high-resolution version of this figure is included in the supplementary material online~\cite{saf_toolkit_online}.}
    \label{fig:toolkitModel}
\end{sidewaysfigure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Decision Map and its Instruments}
% \assignedto{Patricia}

\paragraph{The Conceptual Elements}
In \Cref{fig:toolkitModel}, the key elements of the DM (coloured in green) are encompassing architecture-related concepts widely adopted in the field, as well as the essential sustainability-related concepts.

The architecture-related concepts include class \texttt{Software Architecture} as the generic \textit{anchor} to the software project under study (or if you wish, the generic placeholder representing the software architecture), and class \texttt{Design Concern} representing the set of architecture design concerns that are being addressed. In addition, a DM may include elements of class \texttt{Feature} (see the bottom and left-hand side of \Cref{fig:toolkitModel}), which according to the ISO/IEC 25010 standard is an aspect or property (functional or non-functional) realized by architecture elements and as such part of the software architecture. 
In the current release of the SAF Toolkit, a DM can be designed to illustrate design concerns that may address both \texttt{Sustainability-related Requirements} (\eg in EV charging services, how to ensure that any type of citizen can easily understand how to charge), and \texttt{Quality Attributes} (\eg usability).

The sustainability-related concepts, in turn, are represented by association class \texttt{Effect Type} and class \texttt{Expected Impact}. The \texttt{Effect Type} represents the type of sustainability effect between a pair of design concerns (\eg the effect between performance and energy efficiency). Such effect can be measured (or designed to be) positive (\ie contributing to sustainability), negative (\ie hindering sustainability) or undecided (\ie if no measures are taken yet and at design-time it is unclear what type of effect will be observed).
The \texttt{Expected Impact}, in turn, represents the sustainability time dimension and is meant to frame if the impact of a certain design concern is immediate (first order), enabling (second order) or systemic (third order). 

\paragraph{The Decision Map}
By focusing on a selected software project, the DM can illustrate the features that should be sustainability aware. As shown in \Cref{fig:DMnotationANDexample}, a DM makes use of a relatively simple visual notation (summarized in \Cref{fig:DMnotationANDexample}.(a)) so that any type of stakeholder, from IT specialists to general decision makers, can use it to reason about (i) the sustainability implications of their design decisions, and about (ii) the decisions' effect on QAs in the short- and longer term.

\begin{figure}[ht!]
    \centering
    \includegraphics[width=1\linewidth]{figures/DM-notationANDfig.pdf}
    \caption{\change{DM visual notation and a simple example}}
    \label{fig:DMnotationANDexample}
\end{figure}

As an example, \Cref{fig:DMnotationANDexample}.(b) shows the DM for a smart lighting software architecture project, and in particular the feature \texttt{customize lightning} and the related network of sustainability effects that such feature is expected to have on various relevant QAs. For example, the feature is expected to have a \textit{positive effect} on energy savings in the environmental Sustainability Dimension (\ie one can avoid electricity waste by tuning lightning to the actual user needs), which in turn would have a \textit{positive effect} on energy costs in the economic Sustainability Dimension (\ie by saving energy one would reduce energy costs, too).

Further, QAs are mapped on the Time Dimension to enable explicit representation of the type of sustainability impacts that they are designed for. In our example in \Cref{fig:DMnotationANDexample}.(b), configurability of lightning to human behavior has proven to enable positive (second order) effects on well being (\eg on sleeping and eating patterns of children) which in turn may have systemic (third order) effects on the need for (and cost of) healthcare.


\paragraph{The guiding Instruments}\label{sec:guidingInstrument}
% \todo{explain the instruments used to produce a DM}

The SAF Toolkit includes a number of instruments that provide guidance for creating a DM. These instruments are the Checklist and the Decision Graph, both described in the following.

\begin{description}
    \item \textbf{The Checklist} provides a list of reflective questions that help guiding the creation of a DM in a systematic way. It mainly focuses on the identification of the most important QAs and design concerns. \Cref{fig:DM-instruments}.(a) shows a fragment of the Checklist with the reflective questions for identifying the main QAs (and the types of related sustainability effects) for the software project being considered.

\begin{figure}[ht!]
    \centering
    \includegraphics[width=\linewidth]{figures/DM-instruments.pdf}
    \caption{DM instruments}
    \label{fig:DM-instruments}
\end{figure}

    \item \textbf{The Decision Graph} provides guidance to classify each QA according to the most relevant Time Dimension. Practically, 
    it helps deciding where each selected Design Concern (DC) should be placed among the three impact levels (\ie immediate or first-order, enabling or second-order, systemic or third-order -- the graph leaves in \Cref{fig:DM-instruments}.(b)). \\
    In particular, the black text in the figure exemplifies the possible interpretations of each impact level; the blue text provides a simple example of possible mappings. As such, if the QA would be \texttt{maintainability}, depending on its definition, its impact could be measured directly in the software system (\eg if defined as the level of modularity of the design), indirectly (\eg if defined as reusability and hence measurable only after the system is reused in new projects), or systemic (\eg if defined as durability and hence measurable in terms of the stability of the deployed system over longer time periods).
\end{description}

\paragraph{Reflections}

\begin{figure*}[ht] 
  \begin{subfigure}[b]{0.45\linewidth}
    \centering
    \includegraphics[width=0.98\linewidth]{figures/dm.nofeatures.drawio.pdf} 
    \caption{DM: only Design Concerns} 
    \label{fig:DM.DC} 
    \vspace{4ex}
  \end{subfigure}%% 
  \begin{subfigure}[b]{0.55\linewidth}
    \centering
    \includegraphics[width=0.98\linewidth]{figures/dm.variants.drawio.pdf} 
    \caption{DM: extension with variability feature} 
    \label{fig:DM.var} 
    \vspace{4ex}
  \end{subfigure}
\vspace{-30pt}
  \caption{\change{Decision Maps. [See notation in Fig.~\ref{fig:DMnotationANDexample}.(a)]}}
  \label{fig:DM.before} 
\end{figure*}

It must be noted, that the DM notation has evolved over the years to address the needs of sustainability-aware software architecture design decision making, thanks to the experience gained via its use in a series of diverse cases provided by external partners, mostly from industry. For example, while the toolkit was created starting in 2015, only in 2020 we introduced the notion of `feature' to make explicit which aspect of a software system would be responsible for which QAs. Accordingly, before 2020 the DM in \Cref{fig:DMnotationANDexample}.(b) was not including any feature and was looking like the one in \Cref{fig:DM.before}.(a)\footnote{Notice that before 2020 also the visual notation for the effect types was different.}. 

As another example, the more recent work reported in \citet{FunkeEtAl_VariabilityFeatures_2023} had to represent the fact that some features can be realized by multiple variants as illustrated in \Cref{fig:DM.before}.(b).

In \Cref{tab:cases} we summarize a list of exemplary cases that we carried out over the years to apply the SAF Toolkit and when needed, improve it according to the lessons we learned. On the right-hand side, we point to when the SAF Toolkit was revised to accommodate needs that we deserved as generally applicable and adding value. In particular, changes to the DM have been: 
\begin{itemize}
    \item In 2017, a case study carried out with the KPMG consultancy company revealed that after carrying out empirical experiments, we could decorate the effect-arrows with labels that would \textbf{illustrate the measured impact} \eg of a quality concern like performance on another quality concern like energy efficiency. As a consequence, we added impact labels to the DM visual notation (see \texttt{comment} in \Cref{fig:DMnotationANDexample}.(a)).
    \item In 2020, we carried out a research project on food security, in particular in resource-constrained environments (like some African countries) were access to software services can help sustainability and equity. We had to model which \textbf{features} were meant to address equity requirements (\eg provide farmers with audio-based access to services in various local dialects) so that all farmers could exploit the opportunities of selling online their products. It must be noted that in the same project, we experimented with modeling with goals in DMs, too, \ie making explicit the \textbf{sustainability goals} that features are meant to realize. While in this specific project this modeling exercise was beneficial, we did not encounter such a modeling need afterwards, hence we did not leverage this in the toolkit yet.
    \item In some other projects between 2020 and 2022, we found it useful to, \eg model design concerns that are in a hierarchical relation (like that existing between quality characteristics and sub-characteristics) or in the form of \textbf{thematic clusters} (like complexity into organisational, technical or social complexity). While such representations could be model kinds of DMs, we consider them as different views. Also in these cases, we did not need to illustrate them in any other project and hence refrained to extend the DM notation.
    \item In 2020-2023 we carried out a yearly winter school attended by both researchers and practitioners. The participants would bring their own case study. Every school edition, we had one case where modeling the DM elements pertaining a \textbf{stakeholder type} would be beneficial (\eg if some quality concerns would pertain producers and some others consumers). While also in this case we refrained from leveraging the \textbf{clustering of concerns} in the standard DM notation, we noted down this experience as a lesson potentially useful for future releases of the toolkit. 
\end{itemize}

\input{90_table_cases_overview}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Sustainability-Quality Model and its Instruments}
% \assignedto{Nelly}

\paragraph{The Conceptual Elements}
In \Cref{fig:toolkitModel}, the key elements of the SQ Model (coloured in blue) are encompassing quality attributes, dependencies among them, and associated metrics. Quality attributes, in turn, are characterized according to the sustainability dimension they belong to.

\paragraph{The SQ Model}
The SQ Model comprises a collection of \texttt{Quality Attributes} (QAs) categorized into four \texttt{Sustainability-Quality Dimensions} (\eg technical dimension includes security, environmental dimension includes energy efficiency). Recognizing the potential interdependencies among QAs and the multidimensional nature of software sustainability, such \texttt{dependencies} can be of two types:

(i) \textit{Inter-dimensional dependencies}, linking a pair of QAs defined across different dimensions (\eg robustness from the technical dimension positively influencing confidentiality in the social dimension).

(ii) \textit{Intra-dimensional dependencies}, where a dependency emerges between two distinct QAs within the same dimension (\eg within the technical dimension, security may depend on reliability).

Moreover, as our SQ model provides support to both identify design concerns and assess QAs of the software architecture, a set of metrics is used for measuring QAs. Similarly, metrics can be defined for sustainability-related requirements, represented as a class inheriting from class Design Concern.

\paragraph{The guiding Instruments}
The SAF Toolkit further includes a number of instruments that provide guidance for the software architect to produce an SQ Model. These are the SQ Model Template and the Interdimensional Dependency Matrix Template, both described in the following.

\begin{description}
    \item \textbf{The SQ Model Template} provides a structured approach to assist software architects in creating their own specific SQ Model. It comprises three well-defined components:
    \begin{itemize}
        \item \textit{Quality Attributes (QA):} A curated list of QAs considered during the design or assessment of sustainability-aware software systems. Each attribute is accompanied by operational definitions delineating its intended purpose.

        \item \textit{Direct Relationships to Sustainability Dimensions: }Explicit mappings between QAs and overarching sustainability dimensions such as economic, environmental, social, and technical.

        \item \textit{Metrics: }Defined to offer a scale and method for measurement, the metrics encompass three types according to the standard ISO/IEC 25010:2011: internal metrics, external metrics, and quality-in-use metrics.
    
    \end{itemize}

    Overall, the template (see \Cref{fig:SQmodel_Zahori} for an example from \cite{FunkeEtAl_VariabilityFeatures_2023}) is structured in a tabular format and consists of five fields: the name of the QA, its definition, the reference to the source of definition, the corresponding sustainability dimension, and a list of metrics.

    Software architects have the flexibility to customize their SQ Model by either starting from a generic SQ Model that consolidates QA definitions from past projects and ISO/IEC 25010-2011 standards \change{and/or} by introducing new QAs not present in the generic model. They can also refine existing definitions and establish corresponding direct relationships.
    Figure \ref{fig:SQmodel_Zahori} lists two QAs: Execution Time
    (ET) and Energy Efficiency (EE) that contribute to technical and environmental dimensions, respectively. Both QAs  were identified as relevant of a specific sub-feature named \textit{variability} \change{in the context of one of our case studies where we analysed a robot process automation tool named Zahori \cite{FunkeEtAl_VariabilityFeatures_2023}}. The metrics for ET and EE are variant specific, both are external metrics.
    
    %Utility for Software Architects:
    The SQ Model template transcends a mere static list of QAs related to sustainability dimensions; it serves as a dynamic toolset for informed decision-making and planning for the future. Through the construction of their specific SQ Models, architects can:
    \begin{itemize}
        \item Identify QAs that are critical to achieving sustainability within specific contexts.
        \item Incorporate sustainability considerations proactively into the software design process, hence fostering innovation and resilience in the face of evolving environmental, economic and social challenges.
    \end{itemize}

\begin{figure}[H]
    \centering
    %\includegraphics[width=\linewidth]{figures/SQ_table_zahori.png}
    \includegraphics[width=\linewidth]{figures/SQ_table_big.pdf}
    \caption{\change{\textbf{The SQ Model} (example taken from \cite{GuldnerEtAl_DevelopmentEvaluation_2024a}). The SQ Model template consists of the table structure (headers). The inserted examples are ET and EE (rows). \\Dimensions: TEC=Technical; ENV=Environmental; ECO=Economic; SOC=Social}}
    \label{fig:SQmodel_Zahori}
\end{figure}
    
 \item \textbf{The Interdimensional Dependency Matrix (DMatrix) Template}\label{sec:DMatrix} constitutes another vital instrument within the SAF toolkit, designed to facilitate software architects in analyzing and managing dependencies among QAs of the SQ Model. 
 The template allows architects to map out dependencies in a clear and organized manner, including instructions for its use and extension. 
 The DMatrix is organized into rows and columns, each representing a specific QA within the sustainability dimensions D1 and D2, respectively. Three matrices, including \texttt{technical-social, technical-economic, and technical-environmental} were created and evaluated through a nichesourcing study, details  can be found at \cite{CondoriFernandez2024-interdepend}. 
An example of the DMatrix template is shown in~\Cref{fig:DMatrix_TECH-ENV}. The content of each cell of the DMatrix indicates the type of the dependency between the corresponding QAs:
 \begin{itemize}
     \item \textit{Positive Dependency:} A positive dependency between two QAs suggests that improvements or changes in one QA are likely to have positive effects on the other QA. For example, enhancing efficiency, that belongs to the technical dimension,  may positively contribute to another QA of the social sustainability dimension like trust. A positive dependency is represented with the symbol "+".
     \item \textit{Negative Dependency:} Conversely, a negative dependency indicates that changes or improvements in one QA may have adverse effects on the other QA. For example, increasing interoperability of the technical dimension may negatively affect another QA of the environmental dimension such as modifiability. A negative dependency is represented with the symbol "-".
     \item \textit{Indeterminate Dependency:} Some cells may contain the value "I" indicating an indeterminate dependency between pairs of QAs from sustainability dimensions D1 and D2, requiring further contextual information to determine whether the dependency is positive or negative.
 \end{itemize}

 
\begin{figure}[H]
    \centering
    \includegraphics[width=0.85\linewidth ]{figures/DM_TECH-ENV.png}
    \caption{\textbf{An example of Interdimensional Dependency Matrix template showing the  dependencies among QAs of the technical and environmental dimensions. Cells coloured in blue can be used to add dependencies for newly identified QAs} (\cite{CondoriFernandez2024-interdepend}).}
    \label{fig:DMatrix_TECH-ENV}
\end{figure}

By examining the content of each cell, software architects can gain insights into the relationships between different QAs across sustainability dimensions. This understanding helps in decision-making processes and identifying potential trade-offs between sustainability concerns.
 
The DMatrix is instrumental in creating \texttt{Decision Maps}. The nature of dependencies identified in the DMatrix, whether positive, negative, or indeterminate, informs the type of effect between SQ concerns relevant for a project during the Decision Map creation process. 
\change{The DM instruments, i.e., the checklist and decision graph (see \Cref{fig:DM-instruments}) guide the toolkit user through the creation process of the DM and applying the DMatrix accordingly. In \Cref{sec:SAFinAction} we bring all the instruments together and show how they are applied in a practical context.}
\end{description}



\paragraph{Reflections}
%\todo{Nelly: add your lessons learned and what is still missing}
The development and application of the SQ Model template and the DMatrix template have underscored the significance of integrating sustainability considerations into software architecture design. By integrating sustainability dimensions alongside QAs, software architects can make informed decisions to promote technical, environmental, social, and economic sustainability in software-intensive systems. Moreover, while we have introduced three matrices focusing on the technical dimension (\ie technical-social, technical-environmental, technical-economic), validation efforts are currently in progress to explore dependencies among QAs across all four sustainability dimensions of SAF. This validation process is becoming increasingly feasible as software companies recognize the significance of addressing sustainability across all dimensions, rather than solely focusing on technical or environmental concerns.

However, there are areas that still demand further attention and development. One such area is the \textit{\textbf{refinement of metrics and measurement techniques}} for evaluating sustainability aspects within software architecture. While existing standards provide a foundation, there is a need for more specific and tailored metrics to capture the unique challenges and opportunities of sustainable software development. 
Another area of improvement is related to the \textit{\textbf{visualization the SQ Model}}. For instance, graph visualization could offer a more intuitive representation of the relationships among quality attributes from different sustainability dimensions, facilitating easier analysis and decision-making. Initial exploration in this direction has been presented in \cite{CIBSE22}.
Moreover, it is important to consider that graph-based models enable the persistence of software project data, supporting storage, retrieval, and manipulation for tracking changes over time. This lays the groundwork for future integration of artificial intelligence (AI) techniques, which can leverage graph data to identify patterns, such as common dependencies, or critical QRs. 

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The SAF Toolkit: Where we are going}\label{sec:SAFfuture}
% \todo{Here we plan the various extensions for the future. 
% In order to realize the plan we will need to solve challenges (which we will describe here as well).}
%\assignedto{Markus} add figure (greyed ones)

As mentioned in~\Cref{sec:bigpicture}, we are working on two main extensions of the SAF Toolkit which we discuss in more details in Sections~\ref{sec:SAF+KPI} and \ref{sec:SAF+SA}. In addition, we explain how we plan to close the loop between architecture design and re-design, and actual measurement and monitoring of the corresponding system implementation, both driven by measures collected via the integration of the Green Lab (in \Cref{sec:greenlab}) and dashboards (in \Cref{sec:dashboard}).

\subsubsection{Integration of KPIs} \label{sec:SAF+KPI}

KPIs are widely used in business organizations to gauge their performance. The integration of the KPI framework \cite{Fatima_2023} with the SAF Toolkit helps embody the notion of sustainability as a software quality in the operational structure of organizations. \Cref{fig:KPImodel} shows the KPI Model, its elements and their relationships with the elements of the SAF Toolkit \ie Sustainability Goal (from DM) and Metric (from SQ Model). 

Business organizations have strategic high-level goals based on the organization's vision and business model. These goals are based on Critical Success Factors (CSFs). 
A CSF defines the critical ingredients that are essential to concretizing and achieving the organizational goal. Achievement of CSFs assumes achievement of success for an organizational goal. This CSF operationalizes the KPI definition and helps motivate the choice of \textit{`what to measure?'} 
These measures can guide the quantification of metrics. 
These metrics can be used to measure the quality requirements in the SQ Model.
With the integration of the KPI framework within the SAF Toolkit, the same metrics can be used to quantify the KPIs representing one or more quality requirements. Hence, the KPI is representative of the quality requirements as a function of the chosen metric(s).

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/KPIextension.pdf}
    \caption{\textbf{KPI Model}. Detailed overview of the envisioned KPI model and its integration into the SAF Toolkit. The figure uses the notation for Unified Modeling Language (UML) defined in ISO/IEC 19501 \cite{ISO_19501_2005}.}
    \label{fig:KPImodel}
\end{figure}

\change{In a daily workflow, the KPI model can be used to formulate context dependent KPIs to monitor the sustainability goals derived by the DM. Once formulated, fitness functions quantify the KPI and check target achievement. 
If targets are not met, the KPI model provides feedback about the modeled design concerns. This feedback triggers appropriate actions (e.g., optimise efficiency of a certain component) in order to influence the selection and implementation of such design decisions.}
This helps organizations create a synergy between their sustainability goals and concrete architecture design decisions through an action-driven approach. Supplemented by actions, organizations can take practical steps to improve the software architecture by integrating sustainability as a quality in a goal-focused and design-centric approach. This semantic structure aids in intentional, reusable, and value-focused data collection. 

% \textbf{SQ Model} helps identify the relevant and possible QAs per dimension and the impacts that each QA might have across dimensions. 
% \textbf{Decision Map} helps identify the inter-QA impacts. As QAs are represented across four sustainability dimensions, these impacts can also be represented across dimensions (\ie intra-dimension and inter-dimension). Based on the type of impact, we can identify dependencies. Hence, KPIs represented as set of QAs (completely or partially) will also have inter-dependencies. It is always important to see how KPIs effect each other \eg improving one KPI value may suppress or amplify another KPI's value because of the above-mentioned inter-dependencies. Hence, having a visualization as a DMatrix complemented by the SQ model can help identify such dependencies. 
% \textbf{Sustainability Dimensions}

\paragraph{Reflections}

A KPI is most useful when it is realized as a single value indicator with a threshold-based target. In this way, a single number can represent the achievement of success. This, however, is an optimistic assumption that has some practical obstacles, requiring a nuanced understanding of the system.

\textit{\textbf{How to model the KPI functions?}}
The biggest challenge with the KPI framework is choosing and developing the function to quantify the KPI by aggregating the chosen metrics. There is a need for knowledge-based evidence for the development of KPIs and their fitness functions. By using expert knowledge, regulatory support and mathematical modeling techniques, value-focused and relevant KPI functions could be developed.


\textit{\textbf{How to evaluate the sustainability impact with dimensionally hybrid metrics?}}
\change{The measures are inherently mono-dimensional while the metrics can be either mono-dimensional or multi-dimensional.}
A KPI is a function of metrics that emerge from or impact one or more sustainability dimensions. 
\change{Identification of the dependencies between KPIs is not possible using the DMatrix due to its support of mapping by dimension pairs only. However, the metrics used in the DMatrix can help identify the inter-dependencies of metrics and possible inter-dependencies of the KPIs using them. }
We hypothesize that identifying and quantifying the sustainability impacts at the metric level can aid in quantifying the sustainability impact of the KPI across different sustainability dimensions. As identified by Hilty \etal \cite{Hilty_2015}, the representation of abstraction and gauging sustainability impact at different abstraction levels is complex. The metrics quantifying one KPI might have inter-dependencies. For instance, improving the value of a technical metric may lower the value of an environmental metric. Further, if a metric itself is dimensionally hybrid (\ie intrinsically impacts multiple dimensions), then these dependencies become more complicated when viewed at a macro-level. Representing the impacts at this macro-level, where KPIs themselves could also be interdependent, can be complex. \change{Empirical studies are needed to classify the KPI and identify their inter-dependencies. Due to their multi-dimensional nature in the future, we may need different types of dependency matrices.} A systems thinking \cite{checkland1999systems} approach is imperative for such impact analysis. 

\subsubsection{Integration of Software Architecture Descriptions} \label{sec:SAF+SA}
%\assignedto{Markus}

According to the Software Architecture ISO/IEC/IEEE 42010 Standard~\cite{ISO_42010_2022}, a software architecture consists of multiple design decisions, as illustrated in~\Cref{fig:42010model}. The SAF Toolkit incorporates this concept into its DM by integrating design concerns with design decisions. The DM aims to model sustainability concerns during the design phase, with these concerns manifesting as actual decisions in the software architecture at a later stage.

Our toolkit includes the concept of features, which must be distinguished from architectural \texttt{design decisions}. A feature is a desirable and externally observable software property \cite{deckers}. As such it satisfies a requirement or represents a design decision~\cite{Apel2009}. Modeling these features allows architects to (re-)assess their decisions and their impact on sustainability during the design, or re-design. \change{For example, \citet{Fatima_2024_sa} discusses an example of a data retention feature for which two possible design decisions are suggested. The design concern pertains to \textit{retention of data}. The design decisions include options about \textit{retention period} and \textit{access control}. The associated features require the implementation of an archiving feature and an access control feature.}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/42010_extension.pdf}
    \caption{\textbf{Software Architecture}. Detailed overview of the Software Architecture ISO/IEC/IEEE 42010 Standard and its integration into the SAF Toolkit. The figure builds upon the notation for Unified Modeling Language (UML) defined in ISO/IEC~19501~\cite{ISO_19501_2005}.}
    \label{fig:42010model}
\end{figure}

The feature itself is \texttt{realised\_by} one or more concrete architectural elements.

To provide a glimpse of the potential of the planned integration of software architecture descriptions into the SAF Toolkit, in~\Cref{fig:42010model} we show an example specific for the  domain of service-oriented systems that we use in an educational context\footnote{One of the author is teaching a Master-level course on Service Oriented Design. There, software engineering competencies are taught on sustainability-focused projects~\cite{Condori_Fernandez2018}.} (see dashed classes in~\Cref{fig:42010model}). As such, a software service corresponds to a specific service-oriented system and its components.
If explicitly modeled, such association would allow us to locate architecture elements in the software architecture and create the necessary mapping between features, decisions, and concerns. Only by introducing this mapping can we accurately evaluate the impact  on sustainability of both the taken decisions and the specific architectural elements.


\paragraph{Reflections}
%\todo{Markus: add here the lessons learned and future plans (if applicable)}
\change{Our goal is to \textbf{\textit{establish traceability}} between architecture elements and their sustainability impacts. We need to understand which elements are responsible for the measured impact and to what extent. Such knowledge will provide us with information on where in the architecture we need to improve. Future direction is needed to frame this traceability as, for example, a reusable catalogue of architecture viewpoints (i.e. "conventions for creating, interpreting, presenting and analysing a view"~\cite{ISO_42010_2022}) or model kinds (i.e. "conventions for model-based view components"~\cite{ISO_42010_2022}). Another possibility would be to build on a definition of sustainability as a quality attribute and, as such, to frame related concerns as architecture perspectives (i.e. "a collection of activities, tactics, and guidelines used to ensure that a system exhibits a particular set of related quality properties that require consideration across a number of the system's architectural views"~\cite{RozanskiWoods_SoftwareSystems_2005}).}

It is worth noting that the newly introduced \textbf{\textit{concept of aspects}} in accordance with the Software Architecture ISO/IEC/IEEE 42010:2022 Standard~\cite{ISO_42010_2022} can include concerns or non-functional properties (cf. \Cref{fig:KPImodel}). 
\change{In other words, aspects are the "\textit{visible} evidence (in an ADs models and views) for how concerns are addressed"~\cite{rich}.}
However, in the current version of the standard, aspects are only linked to properties of interest but are not explicitly linked to features resulting in a missing relationship to the architecture element. Therefore, the notion of aspects cannot yet be linked to the SAF Toolkit. We identify two challenges: 
(i) how can aspects be linked to features? 
(ii) how can we effectively create the necessary traceability as mentioned above?
Tackling both challenges will help us to successfully provide architects with the necessary feedback about which of the taken decision(s) have an impact on which architecture element(s) and therefore on sustainability.


In the context of the KPI model, \textbf{\textit{actions are triggered}} if a KPI does not reach its target. These actions are derived from the metrics quantifying the KPI. These metrics can be used to identify the quality requirement they represent and the associated design decisions. Hence, we can say that the actions can drive the choice of making a certain design decision if sustainability is not achieved over-time. However, as mentioned above, an underlying assumption is to be able to trace the measured impact to architecture elements.

\subsubsection{Integration with the Green Lab} \label{sec:greenlab}
% \assignedto{Ivano}

The Green Lab is the experimental platform developed at Vrije Universiteit Amsterdam for conducting empirical studies on the quality of software, with a special emphasis on its energy efficiency. 
At the time of writing, the Green Lab includes: (i) a cluster of 7 servers with different technical specifications for executing experiments targeting Cloud software, datacenters, and applications executing compute-intensive workloads, such as simulation, machine learning, and scientific computing, (ii) about 20 smartphones and 3 tablets for executing experiments on targeting mobile applications, (iii) 32 Raspberry Pi and 8 Arduino Nano boards to test embedded and IoT software, and (iv) other equipment including GPUs, educational robots, VR headsets, wearables.  
All devices in the Green Lab are equipped with state-of-the-art power monitors/profilers, both hardware and software (\eg Monsoon power monitor, Watts Up Pro Meter, Intel RAPL, INA219).

The Green Lab also provides a set of open-source tools for conducting experiments on the energy efficiency of software. Among them, Experiment Runner~\cite{S2_Group_Experiment_Runner} provides a Python library for collecting low-level measures from the power monitor/profiler, transforming them into higher-level metrics (\eg energy), and persisting them according to an open file format (\eg JSON), depending on the needs of the experiment. 

We are planning to integrate (a custom version of) Experiment Runner in the SAF Toolkit. Specifically, by referring to \Cref{fig:KPImodel}, Experiment Runner will be in charge of (i) empirically collecting concrete measures from a running system/prototype (\eg its average power consumption, CPU usage, exchanged HTTP messages) and (ii) making them available within the KPI model in the form of instances of the \texttt{Measure} concept. Collected measures will then be used to enrich the DM related to the running system. 

\paragraph{Reflections}
We expect that software architects using the DM enriched with the collected measures will have a better view of how the system is faring with respect to its KPIs, and thus the reasoning process of the architects will be more precise and grounded in the concrete characteristics of the system at hand. We are planning a campaign of user studies involving students and practitioners to either substantiate or disprove the just-mentioned expectation. 
% \todo{Ivano: add here the lessons learned and future plans (if applicable)}

% \todo{Here I did not put the challenges, let me know if we need to do this here or in the Discussion. We need to be consistent across all subsections 4.3.x, either we put the challenges in all individual subsections or we put them all in the Discussion.}


\subsubsection{Integration with Monitoring Dashboard} \label{sec:dashboard}
% \assignedto{Ivano}

In this paper, we primarily referred to the SAF Toolkit as a set of tools for supporting the \textit{design} of software-intensive systems with sustainability as a first-class concern.  
However, the interest of software architects and decision makers is not confined to the construction and evolution of a software-intensive system, but rather it is critical to efficiently and reliably \textit{operate} it throughout its complete life time~\cite{fitzgerald2014continuous,van2009continuous}. 
This reflection is not new per se, but, with the advent of the microservices architectural style~\cite{di2019architecting,waseem2021design} and the DevOps~\cite{devops} paradigm, continuously operating a software-intensive system, promptly detecting relevant incidents (\eg faults, performance issues), and diagnosing their potential impact \textit{at runtime} has reached an unprecedented level of importance. 

We believe that sustainability decisions are no exception and that the SAF Toolkit will be a valuable tool for continuously evaluating sustainability decisions (and their direct/indirect impact) at runtime. 
Central to this new line of research is the integration of the SAF Toolkit with a monitoring dashboard. 
In this context, monitoring consists of the collection of runtime metrics (\eg energy consumption, memory/CPU usage, number of DB queries, average service latency) and their analysis to keep the overall quality of the system at acceptable levels~\cite{ebert2016devops}. 
As of today, tens of monitoring tools exist for monitoring systems in the context of DevOps~\cite{JSS_2024}, such as Prometheus\footnote{\url{https://prometheus.io}} or NetData\footnote{\url{https://www.netdata.cloud}}. 
Monitoring platforms, \eg Grafana\footnote{\url{https://grafana.com}} provide dashboarding functionalities for querying the collected measures and graphically visualizing them via interactive tables, histograms, time series graphs, heatmaps, \etc  
Technically, the integration of the SAF Toolkit with a monitoring dashboard will consist of (i) a dedicated connector between the monitoring tool collecting measures at runtime and the dashboard,  (ii) a widget for representing SAF instruments (\eg decision maps) in the dashboard, and (iii) a set of mechanisms for mapping the tool-specific collected measures to elements of the KPI model, and in turn to the visualized SAF instrument. 

\paragraph{Reflections}
Using the SAF Toolkit in combination with a monitoring dashboard will be one of the first steps toward the integration of the architecture decision-making process and DevOps. As such, it will be valuable to expand the SAF Toolkit also with functionalities for helping architects promptly understanding the current situation of the system, identifying architecturally-relevant issues (\eg the presence of performance bottlenecks or energy hotspots), and taking timely decisions about how to communicate and solve them. In this context, the usage of large language models tuned for suggesting architectural solutions/tactics in the context of the SAF Toolkit is a promising research direction that we are planning to pursue in future work.

==> old/05_discussion.tex <==
\section{Discussion and Conclusion}\label{sec:discussion}
% \assignedto{all} \todo{drop bullets and ideas}\\
% \assignedto{Patricia} \todo{finalize}

In this paper, we present the SAF Toolkit, a set of instruments aimed to support architects and design decision makers in modeling sustainability as a software quality property.

In our experience, we identified two main types of stakeholders as target users of the toolkit. The first are \textit{practicing architects and decision markers}: in the many cases we could develop with them, we observed that architects consistently found the toolkit useful, both for novices that are new to sustainability in software architecting, and for experienced architects that are already knowledgeable of the relevance of sustainability-quality concerns in their projects but do not know how to extend their practices to apply it. The second type of target stakeholders are \textit{instructors} that want to teach their students about sustainability in software engineering/architecture: we have years of experience in successfully doing that in master level courses, experience that we have translated in the supplementary on material~\cite{saf_toolkit_online}, like small video tutorials (work in progress) and the checklist. Of course, practitioners willing to train themselves would find this beneficial, too.

When we described the current release of the SAF Toolkit (in~\Cref{sec:SAFnow}) and the extensions we planned (in \Cref{sec:SAFfuture}), we provided some reflections on the lessons learned and points for improvement. 
After over a decade of research in collaboration with industry and continuous improvements, the two instruments of DM and SQ Model in the current toolkit release are quite mature and consolidated into a powerful yet simple support for practitioners that may be both experienced and novices. Yet, we are missing the two extensions introducing instruments at design time (defining sound KPIs and linking sustainability elements with architecture elements other than features), and the two extensions that link the toolkit to a measurement environment (like our Green Lab) and a monitoring and reflection environment (like the integration with data collection and dashboarding).

We also care to go back to the definition of sustainability we provided in~\Cref{sec:background}, and our emphasis on the indivisible dimensions of \textit{sustainability-focus} and of \textit{time}. While time is represented in the DM by means of the mapping on impact levels (immediate, enabling and systemic), such representation is static as a DM is meant to visualize a model in a single point in time. Differently, we can truly assess if a software architecture addresses SQ concerns or is helping achieve a targeted sustainability goal only if we observe (\ie measure and visualize) the trend distributed over a time period. Partially, the integration with the dashboard has the potential to represent measures (hence effects) over time. This however needs major research investments and is a main topic of our future research.


==> old/06_conclusions.tex <==
\section{Conclusion}\label{sec:conclusion}
\assignedto{Patricia}

% Conclusions may be used to restate your hypothesis or research question, restate your major findings, explain the relevance and the added value of your work, highlight any limitations of your study, describe future directions for research and recommendations. 
%
% In some disciplines use of Discussion or 'Conclusion' is interchangeable. It is not mandatory to use both. Please refer to Journal-level guidance for any specific requirements. 



==> old/99_notes.tex <==
% comes from GSMM
%-----------------------------------------------------------
% VU start - init version
%-----------------------------------------------------------
\subsection{Sustainability Assessment Framework (SAF) Toolkit}
To guide decision making towards achieving sustainability from a software architecture perspective, the Sustainability Assessment Framework (SAF) Toolkit \cite{SAF_Toolkit_2022} was developed by the Software and Sustainability~(S2) group at Vrije Universiteit Amsterdam. In the context of our proposed GSMM framework, the application areas of the SAF Toolkit are at design time and contributing to a concrete measurement setup. Beyond the focus on energy efficiency, the SAF reflects on the four sustainability dimensions according to \citet{LagoEtAl_FramingSustainability_2015}: (i)~\emph{Technical} dimension encompasses implementation aspects, as well as concerns related to the evolution, maintenance, and long-term utilization of software-intensive systems; (ii)~\emph{Economic} dimension revolves around business considerations, such as capital investment and profitability; (iii)~\emph{Social} dimension emphasizes the integration of the systems within communities considering their impact on individuals and society; (iv)~\emph{Environmental} dimension extends beyond greenhouse gas emissions and encompasses the broader impacts of software activities on the natural ecosystem. For the GSMM, the environmental dimension aims at addressing ecologic concerns, \ie the resource and energy efficiency of software-intensive systems. The complete SAF Toolkit includes the following components:

\begin{itemize}
    \item \textbf{Decision Maps (DM)} \cite{Lago_DecisionMaps_2019}:
    To frame and illustrate the sustainability-relevant design and quality concerns as well as their expected impact, the visual notation of Decision Maps (DMs) is utilised. The impacts can be further classified into three types: (i)~\emph{Immediate} impacts, referring to immediately observable changes; (ii)~\emph{Enabling} impacts, arising from use over time; and (iii)~\emph{Systemic} impacts, referring to persistent changes and requirements, \eg economic structural changes. A library for the online editor tool draw.io\footnote{draw.io - \url{https://www.drawio.com}} is part of the toolkit, assisting in drawing DMs according to its conforming visual notation.

    \item \textbf{Sustainability-Quality (SQ) Model} \cite{Condori-FernandezEtAl_ActionResearch_2020}:
    To capture consolidated definitions about the identified concerns, the Sustainability-Quality (SQ) Model consists of a collection of Quality Attributes (QAs) categorised into the four sustainability dimensions. The QAs are derived according to the ISO/IEC 25010 Standard~\cite{ISO_25010_2011} and based on QAs identified in past projects~\cite{Condori-FernandezEtAl_ActionResearch_2020}. For instance, \emph{availability} relates to the technical dimension, while \emph{energy efficiency} relates to the environmental dimension. To be measurable, the SQ model operationalizes the identified QAs by assigning a set of metrics and measurements.

    \item \textbf{Dependency Matrices (DMatrix)} \cite{Condori-FernandezLago_CharacterizingContribution_2018}:
    To reveal dependencies between QAs and uncover missing concerns at design time, the DMatrix is used. It helps completing and complementing the created DM for the most relevant sustainability dimensions. For instance, there may be an identifiable inter-dependency between \emph{availability} and \emph{energy efficiency}, whereby high availability in the technical dimension could potentially have a negative impact on energy efficiency in the environmental dimension.

    \item \textbf{Checklist}:
    To enhance the guidance during the creation process of a DM and facilitate the definition of its elements, a practical checklist helps in identifying the required elements. Furthermore, an accompanying \emph{Decision Graph} aids in classifying concerns within each of the four sustainability dimensions, as well as determining their level of impact.
\end{itemize}

\begin{figure*}[htp]
	\centering
	\includegraphics[width=\textwidth]{VU_SQ-model.pdf}
	\caption{Sustainability-Quality (SQ) Model example. \textbf{TEC}=Technical; \textbf{ENV}=Environmental; \textbf{ECO}=Economic; \textbf{SOC}=Social}
	\label{fig:vuSQ}
\end{figure*}

\begin{figure}[htp]
	\centering
	\includegraphics[width=\columnwidth]{VU_DecisionMap.pdf}
	\caption{Decision Map (DM) example}
	\label{fig:vuDM}
\end{figure}


\Cref{fig:vuDM} depicts a practical example of a DM identifying an arbitrary software system and its accompanied feature (example based on \cite{FunkeEtAl_VariabilityFeatures_2023}). As automated regression testing might have a positive impact on the overall test-execution time, we might need to consider a negative environmental impact on the energy efficiency due to higher computational power. Such identified concerns (\ie QAs) are further defined in the SQ model and operationalized by identifying concrete metrics, as shown in \Cref{fig:vuSQ}.

%%%% VU method summary old
\item The \emph{Sustainability Assessment Framework (SAF) Tool\-kit} \cite{SAF_Toolkit_2022} (see \cref{sec:application:SAF}) is a collection of tools intended to facilitate a network of sustainability-quality concerns at the software architecture level. The toolkit was developed by the Software and Sustainability (S2) group at Vrije Universiteit Amsterdam. It provides various tools to define, guide, uncover, and eventually operationalize the quality concerns in form of a concrete measurement plan and report.
\item The \emph{Green Lab} at VU Amsterdam (see \cref{sec:application:GreenLab}) is the experimental platform for conducting empirical studies on the quality of software, with a special emphasis on its energy-efficiency. The Green Lab is independent of the type of software system being measured and researchers have used it for measuring mobile apps~\cite{MOBILESoft_2023}, Web apps~\cite{TSE_2023}, microservice-based software~\cite{ICSOC_2023}, robotic software~\cite{EMSE_2023}, and IoT applications~\cite{EASE_2023}. The Green Lab is supported by several open-source tools, which help researchers in following established guidelines for the design and conduction of measurement-based experiments~\cite{Wohlin2012,shull2007guide}. 
%-----------------------------------------------------------
% VU end
%-----------------------------------------------------------





\begin{table}[ht]
\caption{Sustainability Quality (SQ) Model \newline \textbf{REF} = Reference; Dimensions: \textbf{TEC} = Technical; \textbf{ENV} = Environmental; \textbf{ECO} = Economic; \textbf{SOC} = Social}
    \begin{tabularx}{\textwidth}{|m{50pt}|m{85pt}|m{18pt}|l|l|l|l|X|}
    \hline
    \cellcolor[HTML]{EFEFEF}\textbf{QA} & \cellcolor[HTML]{EFEFEF}\textbf{DEFINITION}                                                 & \cellcolor[HTML]{EFEFEF}\textbf{REF} & \cellcolor[HTML]{D4E1F5}\textbf{TEC}              & \cellcolor[HTML]{D5E8D4}\textbf{ENV}          & \cellcolor[HTML]{F8CECC}\textbf{ECO} & \cellcolor[HTML]{FFFF99}\textbf{SOC} & \cellcolor[HTML]{EFEFEF}\textbf{METRIC/KPI} \\ \hline
    Execution Time (ET)             & the time it takes for Zahori to execute the predefined set of tests; Time (in seconds)      & ?                               & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{X}} &                                                         &                                           &                                         & %\begin{equation}
% \begin{aligned}
% ET_{feature}(variant_{X}) ={}   & ET_{system}(variant_{X}) \\
%                                 & - ET_{system}(baseline)
% \end{aligned}
%\end{equation}                                            
\\ \hline
    Energy Efficiency (EE)          & the total energy consumed by Zahori to execute a predefined set of tests; Energy (in Joule) & ?                                  &                                                         & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{X}} &                                           &                                         & %\begin{equation}
% \begin{aligned}
% EE_{feature}(variant_{X}) ={}   & EE_{system}(variant_{X}) \\
%                                 & - EE_{system}(baseline)  
% \end{aligned}
% \end{equation}                                             
\\ \hline
    
    \end{tabularx}
\label{tab:SQmodel}
\end{table}
